Magnetic Activity Cycles and Rotation in Planet-hosting and Non-hosting Solar-type Stars

We analyze periodicities in radial velocity (RV) measurements and magnetic activity indicators (S-index and BIS) for 767 Gaia RV standard stars to distinguish between stellar activity and planetary signals. Significant RV periods were detected in only 359 of these stars. Rotation and magnetic cycle periods are identified through iterative periodogram analysis. Among stars with confirmed planets, $28.2\%$ exhibit RV signals that coincide with activity indicators, compared to $21.3\%$ among stars without planets; however, statistical tests show this difference is not statistically significant. Several RV signals previously attributed to planets, such as those in HIP7240, HIP28460, and HIP48331, are instead likely caused by stellar activity, emphasising the importance of using multiple diagnostics to assess RV variability. We report rotation periods in 125 stars, including 30 new estimates, and detect magnetic activity cycles in 127 stars, 95 of which are new. We further investigate the relationship between rotation and magnetic cycle periods in the context of stellar dynamo theory. The full sample reveals a continuous distribution in the $P_{\rm rot}/P_{\rm cyc}$, Rossby number diagram, lacking the classical division into active and inactive branches and instead showing a negative slope, in contrast to some earlier studies. Interestingly, stars with planetary companions exhibit a steeper trend (slope of $-1.049 \pm 0.078$) compared to non-hosts ($-0.654 \pm 0.056$), suggesting that the presence of planets may subtly influence the host star's magnetic behaviour.

==> readme <==
Dear Colleagues: 

The final publication layout will be produced by using raa.cls. 
Therefore, we strongly encourage you to prepare your LaTeX manuscript 
with this class file. Please unpack raa-package.tar.gz, it includes 

raa.cls        ---- RAA macro class file for LaTeX2e 
sample.tex     ---- a sample file using raa.cls (LaTeX source) 
sample.ps      ---- the PS file created by sample.tex in referee format  
sample.pdf     ---- the PDF file created by sample.tex in referee format  
readme         ---- this file  
f?.eps         ---- three demo figures used in the LaTeX template source
sample2.tex    ---- a sample file for using raa.bst
sample2_fig?.eps -- two demo figures used in sample2.tex
sample2.pdf    ---- the PDF file created by sample.tex in referee format
sample2.bbl    ---- bibliography file using by sample2.tex
bibtex.bib     ---- an example for bibtex file

natbib.sty     ---- This package reimplements the LaTeX \cite command
natnotes.pdf   ---- Brief reference sheet for Natbib (pdf)
raa.bst        ---- Bibliography style file 

Hope you enjoy the use of this macro. Your suggestions and comments are 
highly welcome. Thanks.

Editorial Office
E-mail:  raa@raa-journal.org

